AMR Parsing with Action-Pointer Transformer

Abstract Meaning Representation parsing is a sentence-to-graph prediction task where target nodes are not explicitly aligned to sentence tokens. However, since graph nodes are semantically based on one or more sentence tokens, implicit alignments can be derived. Transition-based parsers operate over the sentence from left to right, capturing this inductive bias via alignments at the cost of limited expressiveness. In this work, we propose a transition-based system that combines hard-attention over sentences with a target-side action pointer mechanism to decouple source tokens from node representations and address alignments. We model the transitions as well as the pointer mechanism through straightforward modifications within a single Transformer architecture. Parser state and graph structure information are efficiently encoded using attention heads. We show that our action-pointer approach leads to increased expressiveness and attains large gains (+1.6 points) against the best transition-based AMR parser in very similar conditions. While using no graph re-categorization, our single model yields the second best Smatch score on AMR 2.0 (81.8), which is further improved to 83.4 with silver data and ensemble decoding.

==> intro.tex <==
%\begin{figure*}[!ht]
%    \centering
    %\includegraphics[scale=0.5]{APTFig1.png}
%    \includegraphics[scale=0.5]{APTFig1.png}
%   \caption{Source sentence, target actions and AMR graph for the proposed oracle and %the sentences \textit{The boy wants to go to New York} (top, partially parsed) and %\textit{The opinion of the boy} (bottom). Source: non-masked elements in %cross-attention displayed in black, copy cursor as an arrow. Target: attachable node %actions displayed in black, current node to attach to as arrow. Actions %\textrm{RED}uce, \textrm{COPY}, \textrm{L}eft/\textrm{R}ight \textrm{A}rc (label), %\textrm{PRED}ict(label).}
%    \label{fig:amrbasic}
%\end{figure*}

\begin{figure*}[!ht]
    \centering
    \includegraphics[scale=0.5]{figures/ex1_4.pdf}
   \caption{Source sentence, target actions and AMR graph for the sentence \textit{The boy wants to go to New York} (partially parsed). The black arrow marks the current token cursor. Notice that the attachment actions (at steps 5, 9 and 10) explicitly refer to past nodes using the id of the action that created the node. The other participant of the attachment action is implicitly assumed to be the most recently created graph node.}
    \label{fig:ex1}
\end{figure*}

\begin{figure}[!ht]
    \centering
    \includegraphics[scale=0.6]{figures/ex3.pdf}
   \caption{Step-by-step parsing of the sentence \textit{your opinion matters}. The proposed model predicts a sub-graph from a single word (\textrm{thing :ARG1-of opine-01}) and allows attachment to all its nodes.}
    \label{fig:ex2}
\end{figure}

% \begin{figure*}
%     \centering
%     \includegraphics[width=\textwidth]{figures/oracle_example3.pdf}
%     \caption{AMR graph generation following the action sequence from our transition system, for the sentence ``The boy wants to go''. There are 3 types of actions corresponding to nodes (red), edges (blue), and others (black). The action indexes are used as pointer values inside the edge actions to refer nodes.  We show an intermediate parsing state in (a) and the final state in (b), with the red arrow marking the source token cursor position during the scan and partially constructed graphs on the right.}
%     \label{fig:amr_oracle}
% \end{figure*}

Abstract Meaning Representation (AMR) graphs \citep{banarescu2013abstract} are semantic representations expressing \textit{who does what to whom} in one or more sentences.
% A single AMR graph maps to multiple surface representations. 
Nodes in an AMR graph correspond to propbank senses, or word lemmas among others, edges correspond mainly to semantic roles but also include many AMR specific constructs to handle aspects such as quantity, comparisons and temporally. 

From a parsing perspective, AMR\'s main characteristic is that nodes and edges are only loosely related to the surface symbols. This makes it considerably more complex than e.g. dependency or constituency parsing and closer in format to problems such as code generation from natural language sentences. Unsurprisingly, sequence to sequence models show the best performances in AMR parsing and the introduction of Transformer \cite{vaswani2017attention}-based parsers in 2020 has considerably strengthen state-of-the-art performance\footnotemark\footnotetext{For perspective, scores have jumped $10$ absolute percentage points since 2017 and $3$ in 2020, $4.6$ including this work.}.

AMR graphs are however far from an unstructured sequence to sequence task. Neighbouring nodes are often mapped to neighbouring words, and nodes names can be frequently obtained as easy transformations of (contextualized) surface symbols such lemmas and propbank senses. Previous works have successfully incorporated these inductive biases in different forms such as alignment as latent permutations \cite{lyu2018amr}, manual clustering and normalization of tokens and nodes, henceforth graph recategorization, \cite{lyu2018amr,zhang2019amr,zhang2019broad,cai2020amr} and strong left-to-right constraints through transition-based parsing \cite{ballesteros2017amr,naseem2019rewarding,astudillo2020transition,lee2020pushing}.

Arguably, transition-based AMR parsing approaches have the strongest inductive bias. They are inspired by their dependency parsing counterpart \cite{dyer2015transition}, which requires an oracle, a rule-based teacher, and processes words from left to right by moving tokens from a buffer to a stack. They also currently yield state-of-the art results and show great sample efficienty \cite{astudillo2020transition,lee2020pushing}. 

Despite their success, these models still suffer from limited expressiveness because some of the design principles of the original dependency parser do not transfer well to AMR. In particular, these approaches use the tokens in the stack to refer both to a surface symbol and the node aligned to it. This makes some nodes unattachable, limits both oracle and model performance and necessitates additional rules that increase label sparsity. Furthermore, unlike stack-LSTMs, the recent stack-Transformer does not push partial graph representations into the stack which makes it redundant.

Inspired by the stack-Transformer and the recent sucess of pointer mechanisms in transition systems (CITE CARLOS), in the work we propose the (WE NEED NAME) model, which entails following contributions

\begin{itemize}
\item We introduce a target-side pointer network that, combined with a source side cursor mechanism, provides a strong inductive bias similar to the stack-Transformer without hampering model expressiveness.
\item We create a new state-of-the-art oracle, compatible with the proposed action pointer-network. The oracle processes strictly left-to-right (no swap operation) and has node attachment guarantees.
\item We explore the use of the target-side masks and cursor to encode partial graph representations through message passing.
\item We show that the proposed approach outperforms current state-of-the art by $1.6$ points in AMR2.0 and AMR1.0.
\end{itemize}


==> oracle.tex <==
%\begin{figure*}[t]
%\includegraphics[scale=0.53]{o7-example.pdf}
%\end{figure*}

AMRs are sentence level semantic graphs that abstract away from surface tokens. Specifically, there are no explicit alignments between sentence token and graph nodes. Moreover, multiple nodes in the graph can arise from one token in the sentence. One such example would be the sub-graph corresponding to word 'opinion' in in Figure \ref{fig:oex2} -- it comprises of two nodes 'thing' and 'opine-01'. Such constructs pose a challenge for transition based parsing approaches that rely on left to right scan of the text performing actions over tokens. In particular, these approaches use the tokens to refer both to a surface symbol and the node aligned to it. In the past, transition-based AMR systems have handled this by either collapsing multiple nodes into one \cite{ballesteros2017amr} or dynamically modifying the text, adding extra tokens for additional nodes \cite{guo2018better}. The former makes the internal collapsed nodes unattachable resulting in less than perfect oracle accuracy while latter disrupts the natural sentence context, making it hard to use highly beneficial pre-trained contextual embeddings.

Another common characteristic of transition-based AMR parsers is very long action sequences [we should quantify this in comparison to dependency parsing]. This is largely due to frequent SWAP operations for non-projective attachments and explicit REDUCE operations to allow multiple parents per node \cite{ballesteros2017amr}. Long actions sequence affect the parser efficiency and can also be harder to learn.

Despite these limitations, token level transition actions are desirable due to their left to right bias and explicit word-node alignments, which allows to exploit copy actions and compensates for data sparsity. They make full use of natural sentence context and also lend themselves easily to the use of rich pre-trained contextual embeddings.

In the following, we propose a simple action oracle that elegantly resolves all these issues making single left to right pass over sentence. On modeling side, this oracle is enabled by a novel target side action-pointer mechanism discussed in Section \ref{sec:model}. 

\subsection{Action Pointer Oracle}

Here, we propose a new action oracle that decouples graph nodes from surface token representations while maintaining explicit alignment between the two. It takes a source sentence as input and produces a target action sequence that can be directly translated into a graph. An example of source/target sequences and AMR graph is depicted in Figure \ref{fig:ex1}, decorated with the different mechanisms involved. Unlike traditional transition-based system that model a stack and a buffer, we simply maintains a cursor over the source sentence tokens that only moves from left to right. It separats the token being processed from already processed (left) and unprocessed (right) tokens. At any time step, the current state of the transition system is fully specified by input tokens, cursor position and current action history.

The oracle actions can be divided into three broad categories: 1) actions that move cursor in the sentence 2) actions that create graph node(s) for current cursor position 3)actions that attach the most recently created graph node to any of the existing nodes. The first set only works with the sentence and the last only with the graph nodes, the middle one connects the two. 

After a node creation action is performed, all its attachments to the existing nodes are done before performing any other actions. Note that any number of node creation or attachment actions can be performed for the same cursor position. Allowing for multiple nodes and arcs, even the entire graph if necessary, from a single source token. This provides a formal guarantee that the oracle can produce all trees while allowing efficient use of copy mechanisms that generate nodes from surface tokens. This in turn reduces data sparsity and increases the models sample efficiency. AMR nodes are drawn from a small fixed vocabulary or are simple transformations of surface symbols, such token copies, as token name or verb lemmas along sometimes with propbank senses. 

Previous works represent nodes by the source tokens aligned to them, which limits oracle expressiveness. Here we utilize instead the target side action history to represent graph nodes. In particular, the actions that produce graph nodes are also used to refer to those nodes for future attachment, obviating the need for separate graph representation while also breaking strong coupling between tokens and nodes.

To allow drawing non-projective arcs, attachment operations i.e. LA and RA, are decorated with the id of the target node (index of the actions that generated the node). The source of the attachment is always the most recently generated node. This mechanism removes the need for the expensive \textrm{SWAP} action used in previous works producing a strictly left-to-right parser.

Below is the list of oracle actions along with their description:

\hline
\begin{itemize}
    \item \textbf{SHIFT:} moves cursor one position to the right. 
    \item \textbf{REDUCE:} a special case of SHIFT used when cursor is moved without performing any actions At current position. 
    \item \textbf{MERGE:} saves current token to be merged with the next and moves the cursor one position to the right. 
\end{itemize}   
\begin{itemize}
    \hline
    \item \textbf{PRED:} Predicts an AMR node for current token position from a vocabulary of nodes. 
    \item \textbf{COPY:} Predicts an AMR node by copying from the token at current cursor position. There are two versions of this actions, COPY\_LEMMA that just copies over the lemma of the token and COPY\_SENSE01 that copied over the lemma with a -01 sense number. 
    \item \textbf{ENTITY:} This action produces a sub-graph with an entity label. Since nodes a represented by actions, the whole sub-graph has only one action representing it. This is an example where multiple nodes get collapsed. We only used it in the cases where internal collapsed nodes have no external attachments, such as named entities.
\end{itemize}   
\begin{itemize}
    \hline
    \item \textbf{LA(id,label):} 
    \item \textbf{RA(id,label):} 
\end{itemize}
     

%    \end{tabular}

%   \caption{Caption}
%   \label{tab:my_label}
%\end{table}

Similar to the past work, the proposed oracle relies on word-to-node alignments that are not part of the gold annotations. We use the combination of rules based JAMR alignments \cite{xx} and EM based alignments of \cite{xx} as proposed by \cite{xx}. 


==> oracle2.tex <==


%\begin{figure*}[t]
%\includegraphics[scale=0.53]{o7-example.pdf}
%\end{figure*}

% overview
% general pipeline of the graph generation
% -->
% limitations of transition-based approaches
% 1) tie source tokens with words
% 2) long action sequence with SWAP
% 2)* this is solved by the graph-based approaches, but it requires several modules, and not having explicit alignment between the graph and the source
% (above is another approach)
% -->
% We propose a transition system that combine both, with a unified transition system that addresses the limitations, and is flexible
% ---

% ~~general solution of the problem~~  (moved to later)
% limitations of the transition-based approaches
Transition-based parsing approaches have been extensively applied to AMR parsing \citep{ballesteros2017amr, buys2017robust, guo2018better, naseem2019rewarding, astudillo2020transition, lee2020pushing} and currently attain state-of-the-art performance \cite{astudillo2020transition, lee2020pushing}. These approaches derive from the original transition-based algorithm \citep{nivre2008algorithms} for dependency parsing and thus suffer certain limitations when extended to AMR graphs. AMRs abstract away from surface tokens and nodes are not explicitly aligned to surface symbols. There are however clear cues that relate surface symbols with one or more graph nodes. Nodes names are frequently copies of words, their lemmas or assigned probank frames, see Figure~\ref{fig:ex1}. Furthermore, often multiple nodes are semantically or lexically related to one surface symbol such as ``thing'' and ``opine-01''  to ``opinion'' in Figure~\ref{fig:ex2}. Being able to exploit these cues is central to performance and sample efficiency.

The dependency parsing models derive node representations from surface symbols and implicitly align every word with only one node. This alignment is not only important for inductive biases, but is also the mechanism through which nodes can be referred to when creating edges. While not a problem in dependency parsing, this impedes the needed one to many alignments required in AMR. Previous attempts to address this issue introduce actions that collapse multiple nodes into one \cite{ballesteros2017amr, naseem2019rewarding, astudillo2020transition} making some nodes unreachable by graph edges, or dynamically add extra tokens for additional nodes \cite{guo2018better}. These solutions required additional actions that increased label sparsity. More importantly, many of these works, including the most performant ones, were unable to fully recover the gold graphs due to unreachable nodes.

% First, different from dependency trees where sentence tokens also act as nodes, AMR abstracts away from surface tokens with node concepts taking different forms and no explicit alignments.
% % One salient aspect is that the sentence tokens also act as nodes in dependency trees, whereas AMRs are sentence level semantic graphs that abstract away from surface tokens, with node concepts differing from source tokens and no explicit alignments. 
% Multiple nodes could also arise from one token in the sentence, as shown in the example in Figure~\ref{}, where the sub-graph of nodes ``thing'' and ``opine-01'' both correspond to the word ``opinion''.
% Such constructs pose a challenge for transition-based approaches, which use tokens to refer both to a source surface symbol and the node concept aligned to it. Previous transition-based AMR systems attempted to handle this by either collapsing multiple nodes into one \cite{ballesteros2017amr} or dynamically modifying the text, adding extra tokens for additional nodes \cite{guo2018better}, but these solutions are far from perfect as the former makes the internal collapsed nodes unattachable, and the latter disrupts the natural sentence context, making it hard to use highly beneficial pre-trained contextual embeddings.


%  (\note{Tahira: we should quantify this in comparison to dependency parsing})

% RAMON: Remove this, what is it? "and explicit $\reduce$ operations needed for multiple parents per node \citep{ballesteros2017amr}."

Another drawback of the current transition-based approaches to AMR parsing is the need for very long action sequences. Unlike dependency parsing, the length of the target action sequence is not bound by twice the token sequence length plus one. The $\swap$ action \citep{nivre2009non}, which moves words from the stack back for the buffer is needed for non-projective attachments, creates very long action sequences in AMR and even stopping condition problems. Moreover, AMR allows multiple parents per node, this requires explicit $\REDUCE$ actions making the sequences even longer. Long action sequences affect decoding speed, moving tokens back to the buffer also breaks the strictly left-to-right processing condition, making learning harder.

%Despite these limitations, introduction of the stack-Transformer approach \cite{astudillo2020transition,lee2020pushing}, showed that improvements on the modeling side can compensate for many of this deficiencies and yield state-of-the-art results.

% motivation: we propose a transition-system that solves the limitations
Given the above limitations, we propose a framework that addresses these issues by combining elements of transition-based parsing and graph-generation approaches. At high level, similar to \cite{astudillo2020transition}, parsing is modeled as sequence to sequence problem, where sentence tokens are the source and action sequence is the target. Instead of stack and buffer, a cursor is maintained over source sentence modeled via cross-attention mechanism of sequence to sequence transformers. On target side, we introduce a novel way of modeling graph nodes -- the target side actions that generate nodes are also used as node representation. Creation of edges is controlled by a pointer mechanism following \cite{ma-etal-2018-stack,fernandez-gonzalez-gomez-rodriguez-2020-transition}. This yields transitions that process the sentence in strict left-to-right fashion, can generate an entire subgraph from a single token and has no attachment restrictions. This yields

%, similar to the graph-based approaches. Finally, we pack our system with a unified representation of node concepts, edge connections, edge labels, and other transitions that can be learned efficiently with a single Transformer-based model.    


% we propose a transition system that is more flexible to deal with all these limitations.... also borrowed from graph-based approaches.

% like other transition-based approaches, our learning and inference framework can be illustrated by figure xxx, with the action sequence serving as the direct learning objective for AMR graphs.

% our transition-system has the following advantages:
% - ... dealing with reentrancy naturally
% - ... efficiency: with pointers
% - ... flexibility: free graph generation, self-loop, multi-edges, all fine
% - it is not limited to AMR graph; general to any text-to-graph generation

% AMRs are sentence level semantic graphs that abstract away from surface tokens. Specifically, there are no explicit alignments between sentence token and graph nodes. Moreover, multiple nodes in the graph can arise from one token in the sentence. One such example would be the sub-graph corresponding to word 'opinion' in in Figure \ref{fig:oex2} -- it comprises of two nodes 'thing' and 'opine-01'. Such constructs pose a challenge for transition based parsing approaches that rely on left to right scan of the text performing actions over tokens. In particular, these approaches use the tokens to refer both to a surface symbol and the node aligned to it. In the past, transition-based AMR systems have handled this by either collapsing multiple nodes into one \cite{ballesteros2017amr} or dynamically modifying the text, adding extra tokens for additional nodes \cite{guo2018better}. The former makes the internal collapsed nodes unattachable resulting in less than perfect oracle accuracy while latter disrupts the natural sentence context, making it hard to use highly beneficial pre-trained contextual embeddings.

% Another common characteristic of transition-based AMR parsers is very long action sequences [we should quantify this in comparison to dependency parsing]. This is largely due to frequent SWAP operations for non-projective attachments and explicit REDUCE operations to allow multiple parents per node \cite{ballesteros2017amr}. Long actions sequence affect the parser efficiency and can also be harder to learn.

% Despite these limitations, token level transition actions are desirable due to their left to right bias and explicit word-node alignments, which allows to exploit copy actions and compensates for data sparsity. They make full use of natural sentence context and also lend themselves easily to the use of rich pre-trained contextual embeddings.

% In the following, we propose a simple action oracle that elegantly resolves all these issues making single left to right pass over sentence. On modeling side, this oracle is enabled by a novel target side action-pointer mechanism discussed in Section \ref{sec:model}. 



==> related_work.tex <==
%AMRs are essentially labeled directed acyclic graphs (DAGs) whose generation relies on certain linearization. Although graph traversal algorithms such as breadth-first and depth-first search orders are used in approaches directly predicting graph nodes \citep{zhang2019amr, cai2020amr}, another prominent way is to describe the generative process coupled with the source tokens via sequential actions following a transition system, converting the graph generation problem to an action sequence generation problem, as is the case in transition-based parsing approaches \citep{ballesteros2017amr, buys2017robust, astudillo2020transition}. The latter has the advantage of explicit node-word alignments in left-to-right processing, which allows to exploit local graph-sentence relations and compensates for data sparsity, establishing the current state-of-the-art for AMR parsing \citep{astudillo2020transition}.

A comparison with other transition-based approaches for AMR parsing can be found in the motivation, Section~\ref{section:oracle2}.

Regarding other high performing approaches for AMR parsing, 

% advantage of graph-based approaches
Note that this is not an issue with graph-based approaches \citep{zhang2019amr, cai2020amr}, as they generate edge connections directly by comparing previous nodes that are not restricted to the stack and buffer structure, although they often require separate modules for different graph sub-tasks such as node labels, edge connections, and edge labels.



AMR parsing lies in the intersection of semantic parsing and graph generation, thus the majority of existing approaches are built upon techniques from these two fields.
%% transition-based approach
Transition-based approaches \citep{wang2016camr, damonte2016incremental, ballesteros2017amr, wang2017getting, guo2018better, liu2018amr, naseem2019rewarding, astudillo2020transition} closely follow the transition-based parsing algorithm used for dependency parsing, but introduce various extensions in the transition system to account for the extra complexity in AMR such as semantic node concepts %different from the sentence words
, named entity recognition, reentrancies, etc. In particular, the reentrancy in the graph is usually dealt with a swap-transition \citep{ballesteros2017amr, astudillo2020transition} to account for the restriction that an arc could only be built between adjacent words on top of the stack, which limits the efficiency of the algorithm.
%% connection to our approach
Our approach shares the similarity with the transition-based approaches in that we also reduce the parsing problem to learning a sequence of transitions, but we moved away from the strict transition-based algorithm to redesign a special system more directly for graph generation with the help of the pointer mechanism for long distance arcs, which is more efficient and flexible.
%% a similar transition system (no pointer, uses shallow different classifiers)
Note that \citet{vilares2018transition} proposed a similar system but they did not use pointers and relied on pipelined feature-based classifiers.


% Methods that inherit ideas from traditional semantic parsing are the transition-based approaches,
% ...since the nodes are floating...
% ... non-projective/reentry, so need to swap... and the problem reduces to learning the actions...

%% graph-based approach
Another category of AMR parsing approaches \citep{cai2019core, zhang2019amr, cai2020amr} treat the problem more as a conditional graph generation task with less focus on the semantic relation between the graph and the sentence. Like general graph generation methods \citep{li2018learning, you2018graphrnn, liao2019efficient}, nodes and edges are generated alternatively, where edges are usually built by comparing node representations with attention mechanisms. Graph structures are often considered to calculate the intermediate node representations via graph neural networks \citep{li2018learning}.
%% connection to our approach
Our approach is also similar to the graph-based approaches in terms of how we generate edges via attention and pointers, and how we use the intermediate graph structural information to facilitate the node representation learning. However, we hybrid the general sequence-to-graph transduction diagram with a transition system that operates on source tokens, injecting direct semantic relations between source tokens and AMR graph parts. Furthermore, instead of having different modules for either node or edge generation \citep{zhang2019amr, cai2020amr}, we integrate the whole pipeline within a single Transformer decoder for multitasking which proves to be effective.

% moving away from the semantic 
% ... general graph generation approach... often involves graph embedding gnn...
% ... amr parsing with pipelines, for concept and edge...

%% in Introduction
% There are many approaches for AMR parsing, mostly transition-based or graph-based are performing really well...
% Both of the transition-based approaches and the graph-based approaches have been proven very effective pushing the previous state-of-the-art AMR parsing performances.
% We propose a hybrid approach that combines ideas from both tracks, where we design a special transition system based on the source sentence that considers the AMR-source semantic relations, but with transition rules following general graph generation procedures, with the help of the pointer mechanism embedded in the target-side self-attention.
% We ... structural information...
% and ... graph embedding ...

%% seq-to-seq
Other approaches outside of the above two categories also exist, such as \citet{van2017neural, xu2020improving} where the AMR graphs are directly linearized in their penman notation and learned with seq-to-seq models.
% All of these approaches involve transforming the graph structure into some linearized form...
% Simplest one is just to simply linearize to tokens in the graph text...
%% additional techniques, that can be applied to our approach
To further improve the AMR parsing quality, self-learning \citep{lee2020pushing} and pre-training \citep{xu2020improving} approaches that rely on extra data are proposed as well. These techniques are orthogonal to our method and can be applied to boost our performance.

